Best-Effort FPGA Programming: A Few Steps Can Go a Long Way

FPGA-based heterogeneous architectures provide programmers with the ability to customize their hardware accelerators for flexible acceleration of many workloads. Nonetheless, such advantages come at the cost of sacrificing programmability. FPGA vendors and researchers attempt to improve the programmability through high-level synthesis (HLS) technologies that can directly generate hardware circuits from high-level language descriptions. However, reading through recent publications on FPGA designs using HLS, one often gets the impression that FPGA programming is still hard in that it leaves programmers to explore a very large design space with many possible combinations of HLS optimization strategies. In this paper we make two important observations and contributions. First, we demonstrate a rather surprising result: FPGA programming can be made easy by following a simple best-effort guideline of five refinement steps using HLS. We show that for a broad class of accelerator benchmarks from MachSuite, the proposed best-effort guideline improves the FPGA accelerator performance by 42-29,030x. Compared to the baseline CPU performance, the FPGA accelerator performance is improved from an average 292.5x slowdown to an average 34.4x speedup. Moreover, we show that the refinement steps in the best-effort guideline, consisting of explicit data caching, customized pipelining, processing element duplication, computation/communication overlapping and scratchpad reorganization, correspond well to the best practice guidelines for multicore CPU programming. Although our best-effort guideline may not always lead to the optimal solution, it substantially simplifies the FPGA programming effort, and will greatly support the wide adoption of FPGA-based acceleration by the software programming community.

==> TBL/caching_breakdown.tex <==
\begin{table}[h]
\centering
\caption{Normalized breakdown times after caching.}
\label{tab:caching_breakdown}
{\scriptsize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Benchmark & PCIe    & DRAM    & Compute & Overall & Compute Pct. \\ \hline
AES       & 2.2E-03 & 0.12    & 15.0    & 15.1    & 99\%         \\ \hline
BFS       & 0.8     & 0.97    & 6.2     & 8.0     & 78\%         \\ \hline
GEMM      & 6.0E-04 & 2.4E-02 & 10.8    & 10.8    & 99\%         \\ \hline
KMP       & 5.9E-02 & 1.56    & 22.2    & 23.9    & 93\%         \\ \hline
NW        & 1.5E-03 & 4.2E-02 & 6.1     & 6.2     & 99\%         \\ \hline
SORT      & 4.9E-03 & 7.0E-02 & 3.7     & 3.7     & 98\%         \\ \hline
SPMV      & 1.3     & 6.40    & 70.2    & 77.8    & 90\%         \\ \hline
VITERBI   & 1.4E-02 & 0.22    & 36.7    & 37.0    & 99\%         \\ \hline
\end{tabular}
}
\end{table}

==> TBL/caching_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Comparison of execution time in different caching sizes.}
\label{tab:caching_res}
{\scriptsize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Benchmark & No Caching & 4KB  & 64KB & 1MB  & Ideal \\ \hline
AES       & 392.9      & 16.2 & 15.2 & 15.1 & 15.1  \\ \hline
BFS       & 220.8      & 8.0  & 8.0  & 8.0  & 7.9   \\ \hline
GEMM      & 70.2       & 11.0 & 10.8 & 10.8 & 10.8  \\ \hline
KMP       & 765.0      & 23.9 & 23.9 & 23.9 & 23.9  \\ \hline
NW        & 91.8       & 6.2  & 6.2  & 6.2  & 6.2   \\ \hline
SORT      & 99.7       & N/A  & N/A  & 3.7  & 3.7   \\ \hline
SPMV      & 438.3      & 79.4 & 77.9 & 77.8 & 77.8  \\ \hline
VITERBI   & 261.3      & 37.1 & 37.0 & 37.0 & 36.9  \\ \hline
\end{tabular}
}
\end{table}

==> TBL/compute_breakdown.tex <==
\begin{table}[h]
\centering
\caption{Breakdown times after Iteration \#2.}
\label{tab:compute_breakdown}
{\scriptsize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Benchmark & PCIe    & DRAM    & Compute & Overall                 & DRAM Pct. \\ \hline
AES       & 2.2E-03 & 0.12    & 0.09    & 0.21                    & 59\%      \\ \hline
GEMM      & 6.0E-04 & 2.4E-02 & 0.01    & 2.6E-02                 & 91\%      \\ \hline
KMP       & 5.9E-02 & 1.56    & 0.06    & 1.84                    & 85\%      \\ \hline
NW        & 1.5E-03 & 0.04    & 0.01    & 5.5E-02                 & 76\%      \\ \hline
SORT      & 6.3E-03 & 0.07    & 0.05    & \begin{tabular}[c]{@{}l@{}}0.13 (FPGA)\\ 0.16 (CPU)\end{tabular} & 61\%      \\ \hline
SPMV      & 1.3     & 6.40    & 0.10    & 7.75                    & 83\%      \\ \hline
VITERBI   & 1.4E-02 & 0.22    & 0.09    & 0.32                    & 67\%      \\ \hline
\end{tabular}
}
\end{table}

==> TBL/dup_comp.tex <==
\begin{table}[h]
\centering
\caption{Performance improvement on computation lead by PE duplication.}
\label{tab:dup_comp}
{\scriptsize
\begin{tabular}{|l|l|l|l|l|l|}
\hline
Benchmark & 8PE & 16PE & 32PE & 64PE & 128PE \\ \hline
AES       & 1.0 & 2.0  & 4.0  & 7.7  & 15.3  \\ \hline
GEMM      & 1.0 & 2.0  & 3.9  & 7.4  & 13.6  \\ \hline
KMP       & 1.0 & 2.0  & 3.7  & 6.4  &    \\ \hline
NW        & 1.0 & 2.0  & 4.0  & 7.7  &    \\ \hline
SORT      & 1.0 & 1.9  & 3.1  & 4.5  &    \\ \hline
SPMV      & 1.0 & 2.0  & 4.0  & 7.9  &    \\ \hline
VITERBI   & 1.0 & 2.0  & 4.0  & 7.9  & 14.9  \\ \hline
\end{tabular}
}
\end{table}

==> TBL/dup_res.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[h]
\centering
\caption{Performance comparison on different duplication factor.}
\label{tab:dup_res}
{\scriptsize
\begin{tabular}{|l|l|l|l|l|}
\hline
Benchmark & Before Dup & After Dup & Dup Factor & Imprv. \\ \hline
AES       & 15.1       & 0.24      & 128        & 62.5x  \\ \hline
GEMM      & 10.8       & 0.10      & 128        & 107.8x \\ \hline
KMP       & 23.9       & 2.09      & 64         & 11.4x  \\ \hline
NW        & 6.2        & 0.16      & 64         & 38.1x  \\ \hline
SORT      & 3.7        & 0.32      & 64         & 11.6x  \\ \hline
SPMV      & 77.8       & 8.75      & 64         & 8.9x   \\ \hline
VITERBI   & 37.0       & 0.46      & 128        & 81.0x  \\ \hline
\end{tabular}
}
\end{table}

==> TBL/init_breakdown.tex <==
\begin{table}[h]
\centering
\caption{Normalized breakdown times before any refinement.}
\label{tab:init_breakdown}
{\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Benchmark & PCIe & DRAM & Compute & Overall & DRAM Pct. \\ \hline
AES & 2.2E-03 & 377.8 & 15.0 & 392.9 & 96\% \\ \hline
BFS & 0.8 & 213.9 & 6.2 & 220.8 & 97\% \\ \hline
GEMM & 6.0E-04 & 59.5 & 10.8 & 70.2 & 85\% \\ \hline
KMP & 5.9E-02 & 742.7 & 22.2 & 765.0 & 97\% \\ \hline
NW & 1.5E-03 & 85.7 & 6.1 & 91.8 & 93\% \\ \hline
SORT & 4.9E-03 & 96.0 & 3.7 & 99.7 & 96\% \\ \hline
SPMV & 1.3 & 366.9 & 70.2 & 438.3 & 84\% \\ \hline
VITERBI & 1.4E-02 & 224.6 & 36.7 & 261.3 & 86\% \\ \hline
\textit{\textbf{G-Mean}} & \textit{\textbf{1.7E-02}} & \textit{\textbf{198.6}} & \textit{\textbf{13.8}} & \textit{\textbf{216.8}} & \textit{\textbf{92\%}} \\ \hline
\end{tabular}
}
\end{table}

==> TBL/initial.tex <==
\begin{table} [h]
  \centering
  \caption{Slowdown of software-inferred accelerators.}
  {\scriptsize
  \begin{tabular}
    {|l c|l c|l c|} 
    \hline
    {Kernel}&{Slowdown}&{Kernel}&{Slowdown}&{Kernel}&{Slowdown}\\
    \hline \hline
    {AES}&{393x}&{BFS}&{221x}&{GEMM}&{70x}\\
    \hline
    {KMP}&{765x}&{NW}&{92x}&{SORT}&{100x}\\
    \hline
    {SPMV}&{438x}&{VITERBI}&{261x}&{\textbf{\textit{G-Mean}}}&{\textbf{\textit{217x}}}\\
    \hline
  \end{tabular}
  }
\label{tab:init_slowdown}
\end{table}

==> TBL/job_lat.tex <==
\begin{table}[h]
\centering
\caption{Kernel latency scaled to a 320-bit input or output.}
\label{tab:job_lat}
{\scriptsize
\begin{tabular}
    {|l c|l c|l c|} 
    \hline
    {Kernel}&{Cycle}&{Kernel}&{Cycle}&{Kernel}&{Cycle}\\
    \hline \hline
    {AES}&{10190}&{BFS}&{59}&{GEMM}&{1110}\\
    \hline
    {KMP}&{560}&{NW}&{10370}&{SORT}&{4440}\\
    \hline
    {SPMV}&{55}&{VITERBI}&{8973}&{\textbf{\textit{Mean}}}&{\textbf{\textit{4470}}}\\
    \hline
  \end{tabular}
}
\end{table}

==> TBL/lcs_res.tex <==
\begin{table}[h]
\centering
\caption{Performance improvement after L-C-S overlapping.}
\label{tab:lcs_res}
{\scriptsize
\begin{tabular}{|l|l|l|l|}
\hline
Benchmark & Before Opt & After Opt & Performance Improvement \\ \hline
AES       & 0.21       & 0.11      & 1.9x                    \\ \hline
GEMM      & 2.6E-02    & 1.8E-02   & 1.4x                    \\ \hline
KMP       & 1.84       & 1.82      & 1.0x                    \\ \hline
NW        & 5.5E-02    & 2.6E-02   & 2.1x                    \\ \hline
SORT      & 0.29       & 0.23      & 1.2x                    \\ \hline
SPMV      & 7.75       & 4.44      & 1.7x                    \\ \hline
VITERBI   & 0.32       & 0.19      & 1.7x                    \\ \hline
\end{tabular}
}
\end{table}

==> TBL/overall_res.tex <==
\begin{table}[h]
\centering
\caption{Performance improvement after BRAM reorganization.}
\label{tab:overall_res}
{\scriptsize
\begin{tabular}{|l|l|l|}
\hline
Benchmark & Speedup over CPU & Speedup over baseline Acc. \\ \hline \hline
AES       & 73.9x            & 29031x                    \\ \hline
BFS       & 0.2x             & 36x                       \\ \hline
GEMM      & 112.8x           & 7927x                     \\ \hline
KMP       & 10.4x            & 7993x                     \\ \hline
NW        & 65.5x            & 6011x                     \\ \hline
SORT      & 4.7x             & 463x                      \\ \hline
SPMV      & 0.4x             & 181x                      \\ \hline
VITERBI   & 7.5x             & 1969x                     \\ \hline
\end{tabular}
}
\end{table}
